Taiyi: A high-performance CKKS accelerator for Practical Fully Homomorphic Encryption

Fully Homomorphic Encryption (FHE), a novel cryptographic theory enabling computation directly on ciphertext data, offers significant security benefits but is hampered by substantial performance overhead. In recent years, a series of accelerator designs have significantly enhanced the performance of FHE applications, bringing them closer to real-world applicability. However, these accelerators face challenges related to large on-chip memory and area. Additionally, FHE algorithms undergo rapid development, rendering the previous accelerator designs less perfectly adapted to the evolving landscape of optimized FHE applications. In this paper, we conducted a detailed analysis of existing applications with the new FHE method, making two key observations: 1) the bottleneck of FHE applications shifts from NTT to the inner-product operation, and 2) the optimal {\alpha} of KeySwitch changes with the decrease in multiplicative level. Based on these observations, we designed an accelerator named Taiyi, which includes specific hardware for the inner-product operation and optimizes the NTT and BConv operations through algorithmic derivation. A comparative evaluation of Taiyi against previous state-of-the-art designs reveals an average performance improvement of 1.5x and reduces the area overhead by 15.7%.

==> cover-letter.tex <==
We appreciate all reviewers for their insightful comments. All of the revisions are highlighted in blue in the draft.

\textbf{Common Questions:}

\textbf{Q1.} Organization and readability need to improve.

\textbf{A1.} We have reorganized the structure of the background and repolished the paper. 
% We move the introduction of the KLSS method from Section~\ref{sec:back:c} to Section~\ref{sec:back:d}, and we also add the algorithm description for the KLSS method in the Background section.

\textbf{Q2.} Did you use double scaling during execution?

\textbf{A2.} We employ the Double Scale method through DSU component during the bootstrapping operation~(Refer to Section~\ref{sec:design:C} and \ref{sec:res:c}. 
% This work represents a significant advancement and achieves. 
% This revision includes the discussion on the proportion of hardware components in Section~\ref{sec:res:c}. 

\textbf{Q3.} Novelty and architectural contribution.

\textbf{A3.} Please refer the revision in the Section \ref{sec:intro}.
%he novelty and the main architectural contributions can be summarized as follows:
%1. Integrating computer architecture analysis and cryptography algorithm optimizations, we discovered that advancements in cryptographic algorithms can change computational bottlenecks, necessitating additional hardware design enhancements beyond previous key operator acceleration approaches.
%2. We propose dynamic parameters for FHE acceleration, using them throughout the entire application execution process. This approach led to a static compiler that analyzes parameter alpha values, optimizing parallelism design and on-chip storage capacity.
%3. We utilize mature MAC units for complex IP operations. IP computation in KLSS is addressed by enhancing data reuse through optimized data flow and a hierarchical MAC structure (HPIP), enabling efficient to execute IP operations with reduced memory access.
%4. For algorithm optimization of the BConv operation, we propose the BConv fusion method to reduce the BConv operation in the Recover-limbs stages and the ModDown.
% 1. We bridge the computer architecture analysis and the cryptography algorithm optimizations. Previous work believed that by focusing on the design of core operators, excellent acceleration effects can be achieved regardless of improvements in cryptographic algorithms. However, in this work, we found that advancements in cryptographic algorithms can lead to significant changes in the computational hotspots of related applications. This necessitates further improvement and design of hardware structures.
% 2. We provide a new idea for FHE acceleration, which utilizes dynamic parameters throughout the entire application execution process instead of fixed ones. Based on such an idea, we developed a static compiler capable of analyzing the computational complexity of parameter alpha values at various multiplication levels, thereby inferring the optimal alpha at different levels. This design necessitates balancing the parallelism design under different alpha values and optimizing the capacity of on-chip storage in our hardware design process. 
% 3.	We employ mature MAC units to compute complex IP operations. We have observed that non-hotspot IP computation has become a hotspot computation in KLSS. Therefore, this work enhances data reuse opportunities by planning data flow and designing a hierarchical MAC structure(HPIP). This structure enables the accelerator to efficiently perform IP operations.

\textbf{Reviewer A:}

\textbf{Q1.} More details about KLSS in the Background section.

\textbf{A1.} We reorganize the background section and add detailed introductions for KLSS in section~\ref{sec:back:c} of the revision.

\textbf{Q2.} Please show the performance improvement of the Taiyi compared with the KLSS method on the CPU.

\textbf{A2.} We evaluate the execution time of KLSS method on the CPU platform, please refer the Table~\ref{tab:absexetime} in the revision. 
% The results demonstrate that Taiyi achieves an average performance improvement of 197,862 \(\times\).


\textbf{Q3.} Organization and readability need to be improved.

\textbf{A3.} Please refer the Common Questions \textbf{A1.}

\textbf{Q4.} Clarify KLSS method won't increase additional noise.

\textbf{A4.} Please refer the section~\ref{sec:back:c} of the revision.

\textbf{Reviewer B:}

\textbf{Q1.} Clarify the contribution of the BConv optimization.

\textbf{A1.} Please see the Common Questions \textbf{A3}.
% KLSS increases the BConv execution times. To mitigate this, we propose the BConv fusion method, integrating KLSS's final step with the ModDown operation. This integration reduces BConv execution times and minimizes noise increase from approximate values in multiple BConv operations.
% KLSS reduces NTT operation complexity by converting ciphertext groups into smaller ones, requiring sequential BConv operations. However, this increases BConv execution times. To mitigate this, we propose the BConv fusion method, integrating KLSS's final step with the ModDown operation. This integration reduces BConv execution times and minimizes noise increase from approximate values in multiple BConv operations.
% KLSS reduces the NTT operation by converting the ciphertext group into a smaller group, which requires several BConv operations performed sequentially. Consequently, the KLSS method increases the execution times of the BConv operation. To address this, we propose the BConv fusion method, which integrates the final step of KLSS with the ModDown operation. This integration decreases the execution times of the BConv operation and also reduces the noise increase resulting from the approximate values generated by several BConv operations. 

\textbf{Q2.} Explain the overhead of the switch for the different \(\alpha\), and how to pick the optimal values.

\textbf{A2.} The process of $\alpha$ switching is fulfilled by compiler and incur no performance overhead. Please refer the revision in Section~\ref{sec:design:d} for detail.
% This process does not incur additional time loss due to the frequent switching of alpha values. When a ciphertext undergoes a keyswitch, the alpha value is selected based on the number of limbs in the ciphertext, and the limbs are then grouped accordingly. During the calculation process, the corresponding ciphertext is simply loaded based on the different limbs. Therefore, no additional switching time is required. It is important to note that the selection of the determined alpha value is performed by a static compiler.

\textbf{Q3.} Low utilization for the compute core.

\textbf{A3.}
% Component utilization may vary in serial mode due to differing call frequencies. However, o
Despite previous implementation of Taiyi, we add a parallel mode (see last paragraph in section \ref{sec:meth}) and further analyze the hardware utilization (see revised section~\ref{sec:res:b}).
% showing average component utilization reaching 48.4\%, with the HP-IP component achieving up to 85.9\% utilization.
% During the execution process of different operators, the utilization of some components may be lower in serial mode due to the varying number of calls they receive within the context of the entire application. However, in this revision, we have updated the utilization analysis in parallel mode. The results demonstrate that the average utilization of components can reach 48.4%, with the HP-IP component achieving a utilization rate as high as 85.9%.

\textbf{Q4.} Adding more details about the simulator.
% for the changes on the top of simFHE.

\textbf{A4.} Refer the revision in the 2nd paragraph of section~\ref{sec:meth}.

\textbf{Q5.} Explain the datapath \text{NTTU} \(\rightarrow\) \text{AUTOU} \(\rightarrow\) \text{HP-IP}.
% Explain the AutoU is performed after the NTT to handle automorphisms in Figure~\ref{fig:overallksw}.

\textbf{A5.} This is an optional path only for bootstrapping, which is not used for \texttt{HMULT}. Please refer to the revised section~\ref{sec:design:C}.


\textbf{Q6.} Does it also follow the double scaling?

\textbf{A6.} Please refer the Common Questions \textbf{A2}.

\textbf{Q7.} Background can be shortened.

\textbf{A7.} Please refer the Common Questions \textbf{A1}.
% \newpage 

\textbf{Reviewer C:}

\textbf{Q1.} Where the benefits come from.

\textbf{A1.} Our performance benefits come from the following aspects:
1) BCONV reduction through a more efficient BCONV fusion mechanism (see Section~\ref{sec:design:C} in the revision).
2) Usage strategy optimization of NTTU to minimize pipeline stalls during the NTTs (see Section~\ref{sec:design:a} in the revision).
3) HPIP significantly improves the computational concurrency for IP and reduces off-chip data access through data reuse (see Section~\ref{sec:hpip} in the revision).
4) The novel dynamic selection scheme for $\alpha$ integrated with the compiler helps to reduce the computational workload(see Section~\ref{sec:design:d} in the revision).

\textbf{Q2.} Remove the Figure~1,2,4 in original paper.

\textbf{A2.} We remove the aforementioned pictures in the revision.

\textbf{Q3.} How does KLSS's arithmetic intensity compare to hybrid key-switching?
% How does the arithmetic intensity of KLSS compare to hybrid key-switching
% Explain KLSS's advantage over the hybrid key switch.

\textbf{A3.} The algorithm's complexity has undergone a significant decrease, significantly reducing the number of NTT calculations. However, the IP and BConv operations increase. Thus, we design the specific HPIP to accelerate IP operations (see Section~\ref{sec:hpip}) and use BConv fusion~(see Section~\ref{sec:bconvfusion}) to reduce the BConv operation. And these optimizations achieve good performance improvement~(see Table~\ref{tab:absexetime}).
% The algorithm's complexity has undergone significant changes, leading to a reduction in the computational load and, consequently, a decrease in the program's execution time. This reduction is primarily achieved by significantly reducing the number of NTT calculations. Additionally, to efficiently calculate IP operations, we utilize data flow planning to reuse the input ciphertext during the IP calculation process. This optimization significantly reduces the number of memory accesses and increases the concurrency of calculations.

\textbf{Q4.} Report absolute performance compared to prior work.

\textbf{A4.} Refer the Table~\ref{tab:absexetime} in the revsion.
% re-evaluated the performance of Taiyi in parallel mode, and the results show a performance improvement of 1.54\(\times\). For specific details, please refer to Section VI of the revised paper.

\textbf{Q5.} Figure~\ref{fig:appbreak} (previous Figure 7) should include the key switch timing breakdowns for total execution.

\textbf{A5.} Please refer the Fig.~\ref{fig:appbreak} of the revision.

\textbf{Q6.} How to overcome memory limitations when executing IP compared to SOTA.
% How to overcome memory limitations without increasing off-chip bandwidth compared to the SOTA.

\textbf{A6.} We utilize data flow planning to reuse the key during the Keyswitch calculation process~(see section~\ref{sec:hpip}). This optimization significantly reduces the memory access times and increases the concurrency of calculations~(see Table~\ref{tab:absexetime}).

\textbf{Q7.} Is there a typo in Fig~\ref{fig:level}~(Previous Fig~8)? 
% The y-axis seems wrong.

\textbf{A7.}  Please refer the Fig.~\ref{fig:level} of the revision.

\textbf{Reviewer D:}

\textbf{Q1.} Clarify the contribution of the NTTU.
% compared with the SHARP.

% \textbf{A1.} Please refer the Reviewer C \textbf{A3}.
We propose an efficient NTTU usage strategy. Our distinct hardware usage and twiddle factor generation strategies effectively eliminated pipeline pauses in the second phase and enhanced the performance of the NTTU~(see Table~\ref{tab:absexetime}) .

\textbf{Q2.} Clarify the architectural contribution of the HPIP

\textbf{A3.} Please refer the Common Question \textbf{A3}.
% We employ mature MAC units to compute complex IP operations. We have observed that non-hotspot IP computation has become a hotspot computation in KLSS. Therefore, this work enhances data reuse opportunities by planning data flow and designing a hierarchical MAC structure(HPIP). This structure enables the accelerator to efficiently perform IP operations.

\textbf{Q3.} Explain the key parameter ($\alpha'$ and $\widetilde{\beta}$).

\textbf{A3.} Please refer Table~\ref{tab:ckkspara} in the revision.
% In this revision, we have specified values such as alpha, where alpha represents the size of the ciphertext space to be converted into the \( R^{T} \) domain in KLSS. A larger $\alpha'$ value necessitates more NTT calculations while ensuring the lower limit of security is met. To strike a balance between performance and correctness, we chose \(\alpha\)'as 4, a value validated in the original paper~\cite{newkey}. Additionally, the \(\widetilde{\beta}\) value is dynamically transformed and is related to the total number of NTT and IP calculations, following the formula \(\frac{L+\alpha}{\alpha}\).

\textbf{Q4.} Please provide the Main memory information.

\textbf{A4.} We utilize HBM as the main memory, with a maximum power consumption of 37W (See Section~\ref{sec:res:b} in the revision).
% During the execution of the ResNet-20 application, it consumes up to 2.47 joules of energy. Please refer to Section~\ref{sec:res:b} in the revision.

\textbf{Q5.} Provide the additional analysis for dnum=2,3,4,5

\textbf{A5.} The overall performance trend of the new and old algorithms is depicted in Table~\ref{tab:reduction}, indicating that the KLSS algorithm did not exhibit significant performance improvement when the \textit{dnum} value was small. As \textit{dnum} approached 6, the overall acceleration effect became more obvious.


\textbf{Q6.} Explain why not increase the number of the EWE.

\textbf{A6.} Please refer the Section~\ref{sec:res:c} of the revision.
% The novel \texttt{HP-IP} component comprises only 10.9\% of the total area, leading to a 74.2\% reduction in area overhead compared to equivalent EWE units with similar parallelism. For more details, please refer to the revision in the paper.
% This efficiency is achieved through the shared utilization of compute units for the same limbs within the \texttt{HP-IP}. 

\textbf{Q7.} Why the memory-intensive IP operation achieves performance improvement in \texttt{HPIP}.

\textbf{A7.} Please refer the Common Question \textbf{A3.}
% The IP operation is memory-intensive. In our design, we reduce memory accesses by sharing ciphertext during calculation with the evaluation key and using batch format for data processing. This allows the high-concurrency IP computing component to achieve excellent acceleration. Small batch memory access requirements can be overlapped by shared computing logic, leading to performance gains.
% The IP operation is a memory-intensive. However, in our design, we effectively reduce the number of memory accesses by sharing ciphertext during calculation with the evaluation key and employing batch format for batch data processing. Therefore, the high-concurrency IP computing component achieves excellent acceleration effects. These small batch memory access requirements can be overlapped by shared computing logic, thereby achieving performance gains.

\textbf{Q8.} The paper seems to not use double scaling.

\textbf{A8.} Please refer the Common Question \textbf{A2.}



